Monotone Circuit Lower Bounds from Robust Sunflowers

Robust sunflowers are a generalization of combinatorial sunflowers that have applications in monotone circuit complexity, DNF sparsification, randomness extractors, and recent advances on the Erd\H{o}s-Rado sunflower conjecture. The recent breakthrough of Alweiss, Lovett, Wu and Zhang gives an improved bound on the maximum size of a $w$-set system that excludes a robust sunflower. In this paper, we use this result to obtain an $\exp(n^{1/2-o(1)})$ lower bound on the monotone circuit size of an explicit $n$-variate monotone function, improving the previous best known $\exp(n^{1/3-o(1)})$ due to Andreev and Harnik and Raz. We also show an $\exp(\Omega(n))$ lower bound on the monotone arithmetic circuit size of a related polynomial. Finally, we introduce a notion of robust clique-sunflowers and use this to prove an $n^{\Omega(k)}$ lower bound on the monotone circuit size of the CLIQUE function for all $k \le n^{1/3-o(1)}$, strengthening the bound of Alon and Boppana.

==> abstract.tex <==
Robust sunflowers (called quasi-sunflowers in \cite{rossman_kclq,gopalan2013dnf,li2018sunflowers} and approximate sunflowers in \cite{lovett2019dnf,lovett2019fromdnf}) are a generalization of sunflowers that are useful in approximating a monotone function by one with few minterms.
For $p,\eps \in (0,1)$, a set system $\mc F$ is a {\em $(p,\eps)$-robust sunflower} if 
\[
  \Pr_{\text{$p$-random subset $R$ of $\bigcup\mc F$}}\Big[\ (\exists S \in \mc F)(S \setminus \textstyle\bigcap\mc F \subseteq R) \ \Big]
  \ge 1 - \eps
\]
where $\bigcup\mc F$ (resp.\ $\bigcap\mc F$) is the union (resp.\ intersection) of all sets in $F$. 
Rossman \cite{rossman_kclq} showed that every $w$-set system of size $\Omega(w\log(1/\eps)/p)^w$ contains a $(p,\eps)$-robust sunflower. In a recent breakthrough, Alweiss, Lovett, Wu and Zhang \cite{alweiss2019improved} obtained a bound $\Omega(\log(w)\log(1/\eps)/p)^{cw}$ for a constant $c \ge 1$, where $c=2$ suffices in general and $c=1$ suffices for any fixed $p$ and $\eps$.

In this paper, we investigate the power of robust sunflowers in proving monotone circuit lower bounds. We show the following results:
\begin{enumerate}[\ \ (i)]
\item
The $k$-clique function on $n$-vertex graphs requires monotone circuit size $n^{\Omega(k)}$ for all $k \le n^{1/3-o(1)}$. (This extends $n^{\Omega(k)}$ lower bounds of Razborov \cite{razborov_boolean_85} and Rossman \cite{rossman_kclq} for $k \le \log n$ and improves an $n^{\Omega(\sqrt k)}$ lower bound of Alon and Boppana \cite{alon_boppana} for $k \le n^{2/3-o(1)}$.)
\item
We match the strongest known $\exp(n^{1/3-o(1)})$ lower bound of Harnik and Raz \cite{HR00} on the monotone circuit size of an explicit $n$-variable monotone function. We also prove an $\exp(\Omega(n))$ lower bound on the monotone arithmetic circuit size of a related polynomial.
\item
We show that improving the constant $c$ to $1$ in the result of Alweiss, Lovett, Wu and Zhang implies an improvement from $n^{1/3-o(1)}$ to $n^{1/2-o(1)}$ in results (i) and (ii).
\end{enumerate}
